Magellan/M2FS and MMT/Hectochelle Spectroscopy of Dwarf Galaxies and Faint Star Clusters within the Galactic Halo

We present spectroscopic data for 16369 stellar targets within and/or toward 38 dwarf spheroidal galaxies and faint star clusters within the Milky Way halo environment. All spectra come from observations with the multi-object, fiber-fed echelle spectrographs M2FS at the Magellan/Clay telescope or Hectochelle at the MMT, reaching a typical limiting magnitude G < 21. Data products include processed spectra from all observations and catalogs listing estimates -- derived from template model fitting -- of line-of-sight velocity (median uncertainty 1.1 km/s) effective temperature (234 K), (base10 logarithm of) surface gravity (0.52 dex in cgs units), [Fe/H] (0.38 dex) and [Mg/Fe] (0.24 dex) abundance ratios. The sample contains multi-epoch measurements for 3720 sources, with up to 15 epochs per source, enabling studies of intrinsic spectroscopic variability. The sample contains 6078 likely red giant stars (based on surface gravity), and 4494 likely members (based on line-of-sight velocity and Gaia-measured proper motion) of the target systems. The number of member stars per individual target system ranges from a few, for the faintest systems, to ~ 850 for the most luminous. For most systems, our new samples extend over wider fields than have previously been observed; of the likely members in our samples, 823 lie beyond twice the projected halflight radius of their host system, and 42 lie beyond 5 Rhalf.

==> compare_previous_offsets.tex <==
\newcommand{\hectovn}{172} 
\newcommand{\hectovfrac}{$0.00\pm 0.00$} 
\newcommand{\hectovsigmaout}{$0.50\pm 0.86$} 
\newcommand{\hectovoffset}{$0.58\pm 0.12$} 
\newcommand{\hectovscale}{$0.00\pm 0.00$} 
\newcommand{\hectoteffn}{172} 
\newcommand{\hectotefffrac}{$0.00\pm 0.00$} 
\newcommand{\hectoteffsigmaout}{$0.98\pm 1.15$} 
\newcommand{\hectoteffoffset}{$102\pm 15$} 
\newcommand{\hectoteffscale}{$0\pm 0$} 
\newcommand{\hectologgn}{172} 
\newcommand{\hectologgfrac}{$0.00\pm 0.00$} 
\newcommand{\hectologgsigmaout}{$-0.66\pm 0.75$} 
\newcommand{\hectologgoffset}{$0.13\pm 0.04$} 
\newcommand{\hectologgscale}{$0.00\pm 0.00$} 
\newcommand{\hectozn}{172} 
\newcommand{\hectozfrac}{$0.00\pm 0.00$} 
\newcommand{\hectozsigmaout}{$-0.65\pm 0.73$} 
\newcommand{\hectozoffset}{$0.00\pm 0.02$} 
\newcommand{\hectozscale}{$0.00\pm 0.00$} 
\newcommand{\hectoalphan}{172} 
\newcommand{\hectoalphafrac}{$0.00\pm 0.00$} 
\newcommand{\hectoalphasigmaout}{$-0.96\pm 0.63$} 
\newcommand{\hectoalphaoffset}{$0.15\pm 0.02$} 
\newcommand{\hectoalphascale}{$0.00\pm 0.00$} 
\newcommand{\walkervn}{1547} 
\newcommand{\walkervfrac}{$0.00\pm 0.00$} 
\newcommand{\walkervsigmaout}{$0.38\pm 0.83$} 
\newcommand{\walkervoffset}{$0.03\pm 0.01$} 
\newcommand{\walkervscale}{$0.00\pm 0.00$} 
\newcommand{\apogeevn}{277} 
\newcommand{\apogeevfrac}{$0.00\pm 0.00$} 
\newcommand{\apogeevsigmaout}{$0.48\pm 0.81$} 
\newcommand{\apogeevoffset}{$-0.09\pm 0.05$} 
\newcommand{\apogeevscale}{$0.00\pm 0.00$} 
\newcommand{\apogeeteffn}{277} 
\newcommand{\apogeetefffrac}{$0.00\pm 0.00$} 
\newcommand{\apogeeteffsigmaout}{$1.06\pm 1.13$} 
\newcommand{\apogeeteffoffset}{$-178\pm 3$} 
\newcommand{\apogeeteffscale}{$0\pm 0$} 
\newcommand{\apogeeloggn}{277} 
\newcommand{\apogeeloggfrac}{$0.00\pm 0.00$} 
\newcommand{\apogeeloggsigmaout}{$-0.73\pm 0.75$} 
\newcommand{\apogeeloggoffset}{$-0.59\pm 0.01$} 
\newcommand{\apogeeloggscale}{$0.00\pm 0.00$} 
\newcommand{\apogeezn}{277} 
\newcommand{\apogeezfrac}{$0.00\pm 0.00$} 
\newcommand{\apogeezsigmaout}{$-0.55\pm 0.73$} 
\newcommand{\apogeezoffset}{$-0.20\pm 0.01$} 
\newcommand{\apogeezscale}{$0.00\pm 0.00$} 
\newcommand{\apogeealphan}{277} 
\newcommand{\apogeealphafrac}{$0.00\pm 0.00$} 
\newcommand{\apogeealphasigmaout}{$-0.84\pm 0.64$} 
\newcommand{\apogeealphaoffset}{$0.02\pm 0.01$} 
\newcommand{\apogeealphascale}{$0.00\pm 0.00$} 
\newcommand{\kirbyteffn}{629} 
\newcommand{\kirbytefffrac}{$0.00\pm 0.00$} 
\newcommand{\kirbyteffsigmaout}{$1.03\pm 1.16$} 
\newcommand{\kirbyteffoffset}{$-64\pm 4$} 
\newcommand{\kirbyteffscale}{$0\pm 0$} 
\newcommand{\kirbyloggn}{629} 
\newcommand{\kirbyloggfrac}{$0.00\pm 0.00$} 
\newcommand{\kirbyloggsigmaout}{$-0.57\pm 0.75$} 
\newcommand{\kirbyloggoffset}{$-0.35\pm 0.03$} 
\newcommand{\kirbyloggscale}{$0.00\pm 0.00$} 
\newcommand{\kirbyzn}{629} 
\newcommand{\kirbyzfrac}{$0.00\pm 0.00$} 
\newcommand{\kirbyzsigmaout}{$-0.73\pm 0.74$} 
\newcommand{\kirbyzoffset}{$-0.08\pm 0.01$} 
\newcommand{\kirbyzscale}{$0.00\pm 0.00$} 
\newcommand{\kirbyalphan}{629} 
\newcommand{\kirbyalphafrac}{$0.00\pm 0.00$} 
\newcommand{\kirbyalphasigmaout}{$-0.89\pm 0.66$} 
\newcommand{\kirbyalphaoffset}{$-0.30\pm 0.16$} 
\newcommand{\kirbyalphascale}{$0.00\pm 0.00$} 
\newcommand{\hthreevn}{765} 
\newcommand{\hthreevfrac}{$0.00\pm 0.00$} 
\newcommand{\hthreevsigmaout}{$0.57\pm 0.85$} 
\newcommand{\hthreevoffset}{$0.17\pm 0.02$} 
\newcommand{\hthreevscale}{$0.00\pm 0.00$} 
\newcommand{\hthreeteffn}{765} 
\newcommand{\hthreetefffrac}{$0.00\pm 0.00$} 
\newcommand{\hthreeteffsigmaout}{$1.07\pm 1.12$} 
\newcommand{\hthreeteffoffset}{$-173\pm 1$} 
\newcommand{\hthreeteffscale}{$0\pm 0$} 
\newcommand{\hthreeloggn}{765} 
\newcommand{\hthreeloggfrac}{$0.00\pm 0.00$} 
\newcommand{\hthreeloggsigmaout}{$-0.62\pm 0.74$} 
\newcommand{\hthreeloggoffset}{$-0.28\pm 0.02$} 
\newcommand{\hthreeloggscale}{$0.00\pm 0.00$} 
\newcommand{\hthreezn}{765} 
\newcommand{\hthreezfrac}{$0.00\pm 0.00$} 
\newcommand{\hthreezsigmaout}{$-0.55\pm 0.77$} 
\newcommand{\hthreezoffset}{$-0.25\pm 0.00$} 
\newcommand{\hthreezscale}{$0.00\pm 0.00$} 
\newcommand{\hthreealphan}{765} 
\newcommand{\hthreealphafrac}{$0.00\pm 0.00$} 
\newcommand{\hthreealphasigmaout}{$-0.81\pm 0.63$} 
\newcommand{\hthreealphaoffset}{$-0.27\pm 0.00$} 
\newcommand{\hthreealphascale}{$0.00\pm 0.00$} 
\newcommand{\ssppvn}{3583} 
\newcommand{\ssppvfrac}{$0.00\pm 0.00$} 
\newcommand{\ssppvsigmaout}{$0.51\pm 0.83$} 
\newcommand{\ssppvoffset}{$0.51\pm 0.02$} 
\newcommand{\ssppvscale}{$0.00\pm 0.00$} 
\newcommand{\ssppteffn}{3583} 
\newcommand{\sspptefffrac}{$0.00\pm 0.00$} 
\newcommand{\ssppteffsigmaout}{$1.25\pm 1.08$} 
\newcommand{\ssppteffoffset}{$-349\pm 1$} 
\newcommand{\ssppteffscale}{$0\pm 0$} 
\newcommand{\sspploggn}{3583} 
\newcommand{\sspploggfrac}{$0.00\pm 0.00$} 
\newcommand{\sspploggsigmaout}{$-0.51\pm 0.73$} 
\newcommand{\sspploggoffset}{$-0.61\pm 0.01$} 
\newcommand{\sspploggscale}{$0.00\pm 0.00$} 
\newcommand{\ssppzn}{3583} 
\newcommand{\ssppzfrac}{$0.00\pm 0.00$} 
\newcommand{\ssppzsigmaout}{$-0.62\pm 0.75$} 
\newcommand{\ssppzoffset}{$-0.39\pm 0.00$} 
\newcommand{\ssppzscale}{$0.00\pm 0.00$} 


==> hecto_obs_table.tex <==
\begin{deluxetable*}{lllllcccl} 
\tablewidth{0pt} 
\tablecaption{Log of MMT/Hectochelle Observations of Galactic Halo Objects \label{tab:hecto_obs_table}} \tablehead{\colhead{Instrument}&\multicolumn{2}{l}{\colhead{Field Center}}&\colhead{UT date\tablenotemark{a}}&\colhead{UT start\tablenotemark{b}}&\colhead{Exp. Time}&\colhead{$N_{\rm exp}$}&\colhead{$N_{\rm target}$}&\colhead{Object}\\ 
&\colhead{$\alpha_{2000}$ [deg.]}&\colhead{$\delta_{2000}$ [deg.]}&&&\colhead{[sec.]}&} 
\startdata 
Hectochelle & $152.064708$ & $+012.349136$ & 2005-04-01 & 05:06:30 &$9079$ & $3$ & $143$ & Leo I\\ 
Hectochelle & $152.064708$ & $+012.349136$ & 2005-04-02 & 06:13:04 &$14400$ & $4$ & $143$ & Leo I\\ 
Hectochelle & $259.425000$ & $+058.049972$ & 2005-04-02 & 10:52:57 &$8700$ & $3$ & $132$ & Draco\\ 
Hectochelle & $152.166792$ & $+012.274975$ & 2006-04-20 & 05:53:41 &$7500$ & $3$ & $135$ & Leo I\\ 
Hectochelle & $152.107875$ & $+012.309992$ & 2006-04-24 & 05:07:09 &$8100$ & $3$ & $135$ & Leo I\\ 
Hectochelle & $168.355875$ & $+022.149333$ & 2006-04-25 & 05:12:38 &$8100$ & $3$ & $114$ & Leo II\\ 
Hectochelle & $260.958333$ & $+057.870000$ & 2006-04-25 & 08:12:45 &$4846$ & $5$ & $107$ & Draco\\ 
Hectochelle & $210.005667$ & $+014.483664$ & 2006-05-08 & 04:24:44 &$5400$ & $3$ & $191$ & Bootes I\\ 
Hectochelle & $260.102667$ & $+057.885250$ & 2007-02-23 & 12:27:48 &$5400$ & $3$ & $120$ & Draco\\ 
Hectochelle & $257.091792$ & $+057.877306$ & 2007-02-26 & 10:03:25 &$5400$ & $3$ & $139$ & Draco\\ 
Hectochelle & $262.915167$ & $+058.382108$ & 2007-02-26 & 12:22:21 &$7200$ & $4$ & $145$ & Draco\\ 
Hectochelle & $152.765458$ & $-001.052389$ & 2007-02-27 & 09:57:01 &$8400$ & $4$ & $203$ & Sextans\\ 
Hectochelle & $259.407542$ & $+057.775056$ & 2007-02-27 & 12:05:59 &$5400$ & $3$ & $89$ & Draco\\ 
Hectochelle & $152.488750$ & $-001.754222$ & 2007-03-01 & 09:09:06 &$6300$ & $3$ & $176$ & Sextans\\ 
Hectochelle & $259.848625$ & $+058.472900$ & 2007-03-02 & 12:03:38 &$9600$ & $4$ & $87$ & Draco\\ 
Hectochelle & $260.162083$ & $+057.467861$ & 2007-03-03 & 11:27:16 &$5400$ & $3$ & $102$ & Draco\\ 
Hectochelle & $259.848625$ & $+058.472900$ & 2007-03-05 & 10:40:06 &$671$ & $1$ & $87$ & Draco\\ 
Hectochelle & $259.848625$ & $+058.472900$ & 2007-03-06 & 10:34:33 &$5400$ & $3$ & $88$ & Draco\\ 
Hectochelle & $260.162083$ & $+057.467861$ & 2007-03-06 & 11:37:38 &$1800$ & $1$ & $99$ & Draco\\ 
Hectochelle & $260.162083$ & $+057.467861$ & 2007-03-09 & 10:34:52 &$5400$ & $3$ & $100$ & Draco\\ 
Hectochelle & $262.915167$ & $+058.382111$ & 2007-03-09 & 12:17:38 &$4500$ & $3$ & $145$ & Draco\\ 
Hectochelle & $257.091792$ & $+057.877306$ & 2007-03-10 & 12:00:31 &$5400$ & $3$ & $137$ & Draco\\ 
Hectochelle & $152.488750$ & $-001.754222$ & 2007-03-11 & 08:22:09 &$8400$ & $4$ & $176$ & Sextans\\ 
Hectochelle & $259.407542$ & $+057.775056$ & 2007-03-11 & 10:56:25 &$7200$ & $4$ & $93$ & Draco\\ 
Hectochelle & $152.102167$ & $+012.306589$ & 2007-03-12 & 08:14:57 &$8100$ & $3$ & $144$ & Leo I\\ 
Hectochelle & $152.102167$ & $+012.306589$ & 2007-04-22 & 05:24:25 &$8100$ & $3$ & $130$ & Leo I\\ 
Hectochelle & $168.355875$ & $+022.149336$ & 2007-04-22 & 08:07:11 &$8100$ & $3$ & $118$ & Leo II\\ 
Hectochelle & $258.601667$ & $+057.479889$ & 2007-04-22 & 10:19:22 &$5400$ & $3$ & $118$ & Draco\\ 
Hectochelle & $261.647292$ & $+058.257119$ & 2007-04-23 & 08:57:21 &$5400$ & $3$ & $73$ & Draco\\ 
Hectochelle & $262.529042$ & $+057.640064$ & 2008-02-24 & 12:05:09 &$6000$ & $5$ & $104$ & Draco\\ 
Hectochelle & $201.977000$ & $+033.568742$ & 2008-02-25 & 08:10:38 &$2400$ & $1$ & $144$ & Canes Venatici I\\ 
Hectochelle & $257.328792$ & $+057.290194$ & 2008-02-25 & 10:42:20 &$3600$ & $3$ & $107$ & Draco\\ 
Hectochelle & $168.357667$ & $+022.142669$ & 2008-02-26 & 06:09:27 &$7200$ & $3$ & $113$ & Leo II\\ 
Hectochelle & $257.987542$ & $+058.300861$ & 2008-02-27 & 11:09:07 &$4500$ & $3$ & $132$ & Draco\\ 
Hectochelle & $260.104208$ & $+057.886569$ & 2008-02-27 & 12:31:44 &$3600$ & $3$ & $52$ & Draco\\ 
Hectochelle & $168.348667$ & $+022.134336$ & 2008-03-01 & 08:32:56 &$7200$ & $3$ & $93$ & Leo II\\ 
Hectochelle & $172.788125$ & $+002.249203$ & 2008-05-28 & 04:52:53 &$7200$ & $3$ & $187$ & Leo V\\ 
Hectochelle & $201.967000$ & $+033.570408$ & 2008-05-28 & 07:56:16 &$9600$ & $4$ & $126$ & Canes Venatici I\\ 
Hectochelle & $227.374917$ & $+067.162283$ & 2008-05-28 & 10:24:58 &$7200$ & $3$ & $180$ & Ursa Minor\\ 
Hectochelle & $151.769000$ & $+015.945714$ & 2008-05-29 & 05:00:13 &$8100$ & $3$ & $212$ & Segue I\\ 
Hectochelle & $227.374917$ & $+067.163956$ & 2008-05-29 & 07:04:40 &$5400$ & $3$ & $200$ & Ursa Minor\\ 
Hectochelle & $227.374917$ & $+067.163956$ & 2008-05-29 & 08:50:53 &$5400$ & $3$ & $169$ & Ursa Minor\\ 
Hectochelle & $229.267375$ & $+067.913025$ & 2008-05-29 & 10:38:01 &$5400$ & $3$ & $133$ & Ursa Minor\\ 
Hectochelle & $172.788125$ & $+002.249203$ & 2008-05-30 & 05:03:08 &$8100$ & $3$ & $192$ & Leo V\\ 
Hectochelle & $226.863417$ & $+066.242697$ & 2008-05-30 & 07:09:33 &$5400$ & $3$ & $98$ & Ursa Minor\\ 
Hectochelle & $229.989583$ & $+068.523278$ & 2008-05-30 & 09:06:22 &$6300$ & $3$ & $102$ & Ursa Minor\\ 
Hectochelle & $227.253333$ & $+067.728906$ & 2008-05-30 & 10:46:37 &$4500$ & $3$ & $114$ & Ursa Minor\\ 
Hectochelle & $034.842208$ & $+020.237775$ & 2008-10-22 & 06:31:37 &$5400$ & $3$ & $205$ & Segue II\\ 
Hectochelle & $034.842208$ & $+020.237775$ & 2008-10-23 & 06:50:45 &$7200$ & $3$ & $191$ & Segue II\\ 
Hectochelle & $034.842208$ & $+020.237775$ & 2008-10-26 & 06:26:44 &$9360$ & $4$ & $207$ & Segue II\\ 
Hectochelle & $172.798917$ & $+002.211903$ & 2009-03-21 & 07:32:24 &$9600$ & $4$ & $214$ & Leo V\\ 
Hectochelle & $257.537542$ & $+057.494728$ & 2009-03-21 & 09:55:05 &$7200$ & $3$ & $116$ & Draco\\ 
Hectochelle & $260.028000$ & $+057.925725$ & 2009-03-21 & 11:35:18 &$4800$ & $2$ & $208$ & Draco\\ 
Hectochelle & $173.209208$ & $-000.597683$ & 2009-03-22 & 07:19:02 &$4800$ & $2$ & $195$ & Leo IV\\ 
Hectochelle & $227.338875$ & $+067.201667$ & 2009-03-23 & 07:56:47 &$9600$ & $4$ & $186$ & Ursa Minor\\ 
Hectochelle & $265.500000$ & $+056.000000$ & 2009-03-23 & 11:03:50 &$9600$ & $4$ & $212$ & Draco\\ 
Hectochelle & $173.209208$ & $-000.597683$ & 2009-03-24 & 09:04:56 &$9600$ & $4$ & $216$ & Leo IV\\ 
Hectochelle & $260.028000$ & $+057.925725$ & 2009-03-24 & 11:39:01 &$7200$ & $4$ & $190$ & Draco\\ 
Hectochelle & $227.295833$ & $+067.214997$ & 2009-03-25 & 11:34:59 &$10800$ & $6$ & $161$ & Ursa Minor\\ 
Hectochelle & $344.646750$ & $+006.039919$ & 2009-10-22 & 05:48:43 &$16200$ & $6$ & $194$ & Pisces II\\ 
Hectochelle & $344.646750$ & $+006.039919$ & 2009-10-23 & 05:55:01 &$13500$ & $5$ & $192$ & Pisces II\\ 
Hectochelle & $034.818125$ & $+020.213939$ & 2009-10-23 & 10:13:20 &$13500$ & $5$ & $189$ & Segue II\\ 
Hectochelle & $320.384167$ & $+019.125331$ & 2009-10-24 & 05:57:27 &$10800$ & $4$ & $155$ & Segue 3\\ 
Hectochelle & $320.373208$ & $+019.162086$ & 2009-10-25 & 05:35:34 &$5400$ & $3$ & $162$ & Segue 3\\ 
Hectochelle & $034.818125$ & $+020.213939$ & 2009-10-26 & 09:54:39 &$13500$ & $5$ & $204$ & Segue II\\ 
Hectochelle & $226.811042$ & $+066.452347$ & 2010-02-05 & 11:20:39 &$8100$ & $3$ & $135$ & Ursa Minor\\ 
Hectochelle & $228.800542$ & $+067.765267$ & 2010-02-06 & 12:03:45 &$8100$ & $3$ & $157$ & Ursa Minor\\ 
Hectochelle & $230.208333$ & $+068.400003$ & 2010-05-15 & 04:56:30 &$7200$ & $4$ & $95$ & Ursa Minor\\ 
Hectochelle & $260.066625$ & $+057.925000$ & 2010-05-15 & 07:23:40 &$6000$ & $4$ & $185$ & Draco\\ 
Hectochelle & $260.066625$ & $+057.925000$ & 2010-05-15 & 09:08:01 &$4500$ & $3$ & $189$ & Draco\\ 
Hectochelle & $258.848000$ & $+057.928333$ & 2010-05-15 & 09:51:15 &$912$ & $1$ & $199$ & Draco\\ 
Hectochelle & $229.291667$ & $+068.199997$ & 2010-05-16 & 04:05:56 &$4500$ & $3$ & $121$ & Ursa Minor\\ 
Hectochelle & $258.848000$ & $+057.928333$ & 2010-05-16 & 05:54:07 &$5400$ & $3$ & $201$ & Draco\\ 
Hectochelle & $261.284292$ & $+057.881669$ & 2010-05-16 & 07:36:37 &$4500$ & $3$ & $197$ & Draco\\ 
Hectochelle & $260.098250$ & $+058.408333$ & 2010-05-16 & 09:13:33 &$4500$ & $3$ & $166$ & Draco\\ 
Hectochelle & $260.048208$ & $+057.415000$ & 2010-05-16 & 10:44:47 &$4500$ & $3$ & $190$ & Draco\\ 
Hectochelle & $260.066625$ & $+057.925000$ & 2011-01-29 & 12:24:10 &$3600$ & $3$ & $201$ & Draco\\ 
Hectochelle & $152.102167$ & $+012.299922$ & 2011-01-30 & 08:26:10 &$9600$ & $4$ & $112$ & Leo I\\ 
Hectochelle & $168.385875$ & $+022.178506$ & 2011-01-30 & 12:16:18 &$12000$ & $5$ & $114$ & Leo II\\ 
Hectochelle & $152.120708$ & $+012.257603$ & 2011-02-05 & 09:26:55 &$9600$ & $4$ & $109$ & Leo I\\ 
Hectochelle & $168.373208$ & $+022.068567$ & 2011-02-05 & 12:33:07 &$9600$ & $4$ & $104$ & Leo II\\ 
Hectochelle & $119.573875$ & $+026.241756$ & 2011-02-06 & 05:49:59 &$9600$ & $4$ & $220$ & Koposov 2\\ 
Hectochelle & $152.110792$ & $+012.265533$ & 2011-02-06 & 08:34:08 &$7200$ & $3$ & $110$ & Leo I\\ 
Hectochelle & $168.384542$ & $+022.180172$ & 2011-02-07 & 07:46:19 &$4800$ & $2$ & $102$ & Leo II\\ 
Hectochelle & $227.321667$ & $+067.210000$ & 2011-04-08 & 07:14:35 &$7200$ & $6$ & $192$ & Ursa Minor\\ 
Hectochelle & $260.066625$ & $+057.925000$ & 2011-05-25 & 07:22:42 &$5400$ & $3$ & $204$ & Draco\\ 
Hectochelle & $260.066625$ & $+057.925000$ & 2011-05-25 & 09:14:22 &$5400$ & $3$ & $196$ & Draco\\ 
Hectochelle & $260.035208$ & $+057.928333$ & 2011-05-25 & 11:05:07 &$4500$ & $4$ & $204$ & Draco\\ 
Hectochelle & $260.733042$ & $+058.042778$ & 2011-05-26 & 07:05:38 &$5400$ & $3$ & $201$ & Draco\\ 
Hectochelle & $259.412708$ & $+057.887222$ & 2011-05-26 & 08:55:43 &$5400$ & $3$ & $206$ & Draco\\ 
Hectochelle & $260.193542$ & $+057.291472$ & 2011-05-26 & 10:55:15 &$4800$ & $4$ & $201$ & Draco\\ 
Hectochelle & $260.082167$ & $+057.872761$ & 2011-05-27 & 07:34:15 &$7200$ & $3$ & $184$ & Draco\\ 
Hectochelle & $260.002417$ & $+058.625167$ & 2011-05-27 & 09:35:30 &$5400$ & $3$ & $195$ & Draco\\ 
Hectochelle & $260.066625$ & $+057.925000$ & 2011-05-27 & 11:01:00 &$3600$ & $3$ & $203$ & Draco\\ 
Hectochelle & $201.967000$ & $+033.570408$ & 2011-05-28 & 07:30:53 &$7200$ & $3$ & $123$ & Canes Venatici I\\ 
Hectochelle & $260.082167$ & $+057.872761$ & 2011-05-28 & 09:53:43 &$7200$ & $3$ & $184$ & Draco\\ 
Hectochelle & $260.072875$ & $+057.911667$ & 2011-05-29 & 07:15:08 &$5400$ & $3$ & $181$ & Draco\\ 
Hectochelle & $259.761000$ & $+057.376675$ & 2011-05-29 & 09:09:01 &$5400$ & $3$ & $200$ & Draco\\ 
Hectochelle & $260.528500$ & $+058.464808$ & 2011-05-29 & 10:45:33 &$4500$ & $3$ & $194$ & Draco\\ 
Hectochelle & $261.726333$ & $+058.491283$ & 2011-05-30 & 10:31:23 &$5400$ & $3$ & $196$ & Draco\\ 
Hectochelle & $258.556292$ & $+057.681358$ & 2011-05-31 & 08:05:43 &$7200$ & $4$ & $199$ & Draco\\ 
Hectochelle & $260.066625$ & $+057.925000$ & 2011-05-31 & 09:37:26 &$3600$ & $3$ & $186$ & Draco\\ 
Hectochelle & $261.726333$ & $+058.491283$ & 2011-05-31 & 10:54:21 &$3600$ & $3$ & $195$ & Draco\\ 
Hectochelle & $227.347458$ & $+067.193328$ & 2012-05-08 & 04:28:25 &$5400$ & $3$ & $190$ & Ursa Minor\\ 
Hectochelle & $227.837000$ & $+067.627883$ & 2012-05-08 & 05:26:56 &$1800$ & $1$ & $120$ & Ursa Minor\\ 
Hectochelle & $227.837000$ & $+067.627883$ & 2012-05-10 & 08:04:10 &$5400$ & $3$ & $119$ & Ursa Minor\\ 
Hectochelle & $151.751875$ & $+015.964456$ & 2012-05-11 & 04:53:51 &$8100$ & $3$ & $196$ & Segue I\\ 
Hectochelle & $153.721250$ & $+017.011431$ & 2012-05-13 & 04:56:54 &$8100$ & $3$ & $212$ & Segue I\\ 
Hectochelle & $168.357250$ & $+022.144200$ & 2013-02-17 & 11:58:34 &$10800$ & $4$ & $87$ & Leo II\\ 
Hectochelle & $168.264458$ & $+022.099272$ & 2013-02-18 & 11:29:09 &$8100$ & $3$ & $84$ & Leo II\\ 
Hectochelle & $153.258583$ & $-001.690311$ & 2015-02-26 & 06:07:25 &$9106$ & $4$ & $205$ & Sextans\\ 
Hectochelle & $210.016375$ & $+014.417925$ & 2015-04-01 & 08:36:53 &$13500$ & $5$ & $199$ & Bootes I\\ 
Hectochelle & $210.011125$ & $+014.419608$ & 2015-04-02 & 07:44:55 &$8100$ & $3$ & $189$ & Bootes I\\ 
Hectochelle & $210.011125$ & $+014.419608$ & 2015-04-06 & 08:08:36 &$8100$ & $3$ & $190$ & Bootes I\\ 
Hectochelle & $033.348792$ & $+036.183422$ & 2015-12-18 & 07:10:13 &$10800$ & $3$ & $197$ & Triangulum II\\ 
Hectochelle & $177.067500$ & $-018.404036$ & 2016-04-27 & 03:14:41 &$10800$ & $3$ & $204$ & Crater II\\ 
Hectochelle & $177.510667$ & $-018.440772$ & 2016-04-30 & 03:16:27 &$8100$ & $3$ & $202$ & Crater II\\ 
Hectochelle & $178.342042$ & $-018.512150$ & 2016-05-11 & 04:59:15 &$8100$ & $3$ & $204$ & Crater II\\ 
Hectochelle & $209.496542$ & $+012.774189$ & 2016-05-11 & 07:42:44 &$8100$ & $3$ & $211$ & Bootes II\\ 
Hectochelle & $226.545917$ & $+066.988333$ & 2016-05-11 & 10:18:38 &$7200$ & $3$ & $180$ & Ursa Minor\\ 
Hectochelle & $209.274292$ & $+026.793333$ & 2016-05-12 & 05:32:36 &$8880$ & $4$ & $174$ & Bootes III\\ 
Hectochelle & $210.040500$ & $+014.493333$ & 2016-05-13 & 04:53:15 &$8100$ & $3$ & $209$ & Bootes I\\ 
Hectochelle & $209.454292$ & $+012.851506$ & 2016-05-13 & 07:30:17 &$8100$ & $3$ & $212$ & Bootes II\\ 
Hectochelle & $227.459542$ & $+067.019522$ & 2016-05-13 & 10:11:40 &$8400$ & $3$ & $176$ & Ursa Minor\\ 
Hectochelle & $209.995750$ & $+014.498103$ & 2016-05-14 & 04:53:57 &$8100$ & $3$ & $206$ & Bootes I\\ 
Hectochelle & $225.865583$ & $+066.447647$ & 2016-05-14 & 10:35:41 &$9148$ & $4$ & $160$ & Ursa Minor\\ 
Hectochelle & $226.786042$ & $+066.272025$ & 2016-06-12 & 05:09:36 &$7200$ & $3$ & $151$ & Ursa Minor\\ 
Hectochelle & $228.372875$ & $+066.114372$ & 2016-06-13 & 05:07:35 &$7200$ & $3$ & $183$ & Ursa Minor\\ 
Hectochelle & $228.425042$ & $+067.018394$ & 2016-06-14 & 05:08:01 &$7200$ & $3$ & $188$ & Ursa Minor\\ 
Hectochelle & $033.348792$ & $+036.185089$ & 2016-10-22 & 05:05:42 &$8100$ & $3$ & $202$ & Triangulum II\\ 
Hectochelle & $344.612417$ & $+005.953031$ & 2016-10-23 & 06:30:53 &$3814$ & $2$ & $204$ & Pisces II\\ 
Hectochelle & $033.348792$ & $+036.185089$ & 2016-10-24 & 05:31:40 &$10800$ & $3$ & $204$ & Triangulum II\\ 
Hectochelle & $344.612417$ & $+005.953031$ & 2016-10-26 & 06:29:19 &$10800$ & $3$ & $204$ & Pisces II\\ 
Hectochelle & $033.348792$ & $+036.185089$ & 2016-10-27 & 06:15:01 &$10800$ & $3$ & $188$ & Triangulum II\\ 
Hectochelle & $033.347167$ & $+036.186100$ & 2016-11-19 & 04:29:09 &$8100$ & $3$ & $202$ & Triangulum II\\ 
Hectochelle & $152.921958$ & $+000.071564$ & 2017-01-30 & 07:49:51 &$8100$ & $3$ & $212$ & Sextans\\ 
Hectochelle & $177.189708$ & $-018.372075$ & 2017-01-30 & 09:05:43 &$10800$ & $4$ & $204$ & Crater II\\ 
Hectochelle & $152.398000$ & $-001.740075$ & 2017-01-31 & 08:22:30 &$8100$ & $3$ & $212$ & Sextans\\ 
Hectochelle & $177.132583$ & $-017.332500$ & 2017-01-31 & 09:33:33 &$10800$ & $3$ & $195$ & Crater II\\ 
Hectochelle & $178.345083$ & $-018.525278$ & 2017-03-01 & 08:32:44 &$5400$ & $2$ & $201$ & Crater II\\ 
Hectochelle & $152.262500$ & $-001.498333$ & 2018-03-10 & 05:18:38 &$7200$ & $3$ & $208$ & Sextans\\ 
Hectochelle & $153.245000$ & $-001.567250$ & 2018-03-19 & 05:32:35 &$10800$ & $4$ & $213$ & Sextans\\ 
Hectochelle & $153.245000$ & $-001.567250$ & 2018-03-20 & 04:54:46 &$7200$ & $3$ & $214$ & Sextans\\ 
Hectochelle & $225.543500$ & $+067.957222$ & 2018-03-20 & 11:22:57 &$8100$ & $3$ & $188$ & Ursa Minor\\ 
Hectochelle & $152.492500$ & $-001.741667$ & 2018-03-21 & 05:00:41 &$10800$ & $4$ & $211$ & Sextans\\ 
Hectochelle & $154.062500$ & $-000.145000$ & 2018-03-22 & 07:22:21 &$5741$ & $3$ & $205$ & Sextans\\ 
Hectochelle & $223.904958$ & $+066.553000$ & 2018-04-05 & 11:19:50 &$5400$ & $3$ & $191$ & Ursa Minor\\ 
Hectochelle & $081.627958$ & $+076.998292$ & 2018-09-21 & 11:15:07 &$6783$ & $3$ & $102$ & KGO 13\\ 
Hectochelle & $081.627958$ & $+076.998292$ & 2018-10-19 & 11:22:36 &$8100$ & $3$ & $99$ & KGO 13\\ 
Hectochelle & $154.117500$ & $-002.464781$ & 2019-02-25 & 06:13:44 &$4800$ & $2$ & $201$ & Sextans\\ 
Hectochelle & $154.117500$ & $-002.464781$ & 2019-02-26 & 07:36:43 &$4800$ & $2$ & $201$ & Sextans\\ 
Hectochelle & $154.667000$ & $-000.238519$ & 2019-02-28 & 07:42:04 &$9600$ & $4$ & $197$ & Sextans\\ 
Hectochelle & $152.639000$ & $-002.250094$ & 2019-03-01 & 06:18:40 &$7200$ & $3$ & $203$ & Sextans\\ 
Hectochelle & $226.676167$ & $+067.405944$ & 2019-03-01 & 08:42:43 &$7200$ & $3$ & $204$ & Ursa Minor\\ 
Hectochelle & $259.847708$ & $+057.889467$ & 2019-03-01 & 11:19:36 &$8100$ & $3$ & $204$ & Draco\\ 
Hectochelle & $153.919167$ & $-000.976861$ & 2019-03-04 & 07:37:39 &$3791$ & $2$ & $196$ & Sextans\\ 
Hectochelle & $228.946708$ & $+067.197136$ & 2019-03-04 & 11:13:51 &$8632$ & $4$ & $200$ & Ursa Minor\\ 
Hectochelle & $224.713250$ & $+067.014519$ & 2019-04-23 & 04:44:45 &$7200$ & $3$ & $204$ & Ursa Minor\\ 
Hectochelle & $229.046792$ & $+067.954750$ & 2019-04-26 & 04:42:08 &$8100$ & $3$ & $205$ & Ursa Minor\\ 
Hectochelle & $258.615792$ & $+057.840347$ & 2019-04-26 & 07:28:10 &$8100$ & $3$ & $204$ & Draco\\ 
Hectochelle & $225.524500$ & $+066.282914$ & 2019-06-24 & 05:25:40 &$7200$ & $3$ & $199$ & Ursa Minor\\ 
Hectochelle & $152.516833$ & $-001.129053$ & 2020-01-31 & 08:11:22 &$7200$ & $3$ & $206$ & Sextans\\ 
Hectochelle & $151.983667$ & $-002.891914$ & 2020-01-31 & 10:00:46 &$4800$ & $2$ & $201$ & Sextans\\ 
Hectochelle & $209.121708$ & $+026.795000$ & 2020-02-02 & 10:18:01 &$8100$ & $3$ & $73$ & Bootes III\\ 
Hectochelle & $132.882792$ & $+063.110717$ & 2020-02-14 & 04:00:16 &$9000$ & $3$ & $195$ & None\\ 
Hectochelle & $158.796917$ & $+052.005428$ & 2020-02-15 & 05:57:27 &$8100$ & $3$ & $141$ & None\\ 
Hectochelle & $151.983667$ & $-002.891914$ & 2020-02-17 & 06:15:04 &$6000$ & $2$ & $201$ & Sextans\\ 
Hectochelle & $210.068375$ & $+014.572592$ & 2020-06-13 & 23:44:25 &$8100$ & $3$ & $198$ & Bootes I\\ 
Hectochelle & $261.218333$ & $+057.370603$ & 2020-06-15 & 05:21:30 &$8100$ & $3$ & $187$ & Draco\\ 
Hectochelle & $259.908833$ & $+057.374917$ & 2020-06-15 & 08:08:00 &$8100$ & $3$ & $199$ & Draco\\ 
Hectochelle & $227.273417$ & $+066.553497$ & 2020-06-16 & 06:17:21 &$8100$ & $3$ & $188$ & Ursa Minor\\ 
Hectochelle & $224.144708$ & $+065.721611$ & 2020-06-17 & 05:17:10 &$7200$ & $3$ & $201$ & Ursa Minor\\ 
Hectochelle & $261.033250$ & $+058.798142$ & 2020-06-17 & 08:42:32 &$9000$ & $3$ & $199$ & Draco\\ 
Hectochelle & $257.359583$ & $+056.479683$ & 2020-06-17 & 10:09:50 &$2700$ & $1$ & $200$ & Draco\\ 
Hectochelle & $261.103667$ & $+057.891556$ & 2020-06-28 & 10:17:21 &$8100$ & $3$ & $203$ & Draco\\ 
Hectochelle & $263.965625$ & $+057.652706$ & 2021-09-29 & 03:51:52 &$8100$ & $3$ & $201$ & Draco\\ 
Hectochelle & $262.224125$ & $+056.812544$ & 2021-10-29 & 02:55:47 &$5400$ & $3$ & $199$ & Draco\\ 
Hectochelle & $262.224125$ & $+056.812544$ & 2021-10-30 & 03:01:21 &$5400$ & $3$ & $199$ & Draco\\ 
Hectochelle & $153.296167$ & $-001.651778$ & 2021-12-12 & 12:01:36 &$9600$ & $4$ & $194$ & Sextans\\ 
Hectochelle & $154.085833$ & $+000.335000$ & 2022-01-05 & 11:28:43 &$10080$ & $4$ & $27$ & Sextans\\ 
Hectochelle & $151.761000$ & $-003.439369$ & 2022-01-06 & 10:27:45 &$9600$ & $4$ & $52$ & Sextans\\ 
Hectochelle & $152.113333$ & $-000.902186$ & 2022-01-06 & 12:58:48 &$5700$ & $3$ & $23$ & Sextans\\ 
Hectochelle & $152.113333$ & $-000.902186$ & 2022-01-07 & 08:41:20 &$4800$ & $2$ & $23$ & Sextans\\ 
Hectochelle & $155.237500$ & $+000.102778$ & 2022-01-07 & 12:13:08 &$11040$ & $4$ & $23$ & Sextans\\ 
Hectochelle & $224.687917$ & $+067.650003$ & 2022-02-26 & 09:33:59 &$8100$ & $3$ & $171$ & Ursa Minor\\ 
Hectochelle & $152.825792$ & $-002.981617$ & 2022-04-05 & 05:00:29 &$9600$ & $4$ & $45$ & Sextans\\ 
Hectochelle & $225.535042$ & $+065.631067$ & 2022-04-05 & 08:29:08 &$10800$ & $4$ & $183$ & Ursa Minor\\ 
Hectochelle & $260.318125$ & $+056.289769$ & 2022-04-05 & 11:17:54 &$8100$ & $3$ & $117$ & Draco\\ 
Hectochelle & $154.378542$ & $-002.426114$ & 2022-04-06 & 05:10:50 &$10800$ & $4$ & $30$ & Sextans\\ 
Hectochelle & $231.043375$ & $+068.266433$ & 2022-04-06 & 07:56:09 &$8100$ & $3$ & $181$ & Ursa Minor\\ 
Hectochelle & $258.828458$ & $+056.363656$ & 2022-04-06 & 11:29:59 &$9900$ & $4$ & $111$ & Draco\\ 
Hectochelle & $260.048542$ & $+057.930325$ & 2022-04-08 & 10:47:50 &$10800$ & $4$ & $170$ & Draco\\ 
Hectochelle & $223.860208$ & $+064.756547$ & 2022-04-09 & 10:59:58 &$11520$ & $4$ & $185$ & Ursa Minor\\ 
Hectochelle & $227.108500$ & $+067.225075$ & 2022-06-20 & 04:18:35 &$2700$ & $1$ & $201$ & Ursa Minor\\ 
\enddata 
\tablenotetext{a}{YYYY-MM-DD format} 
\tablenotetext{b}{Universal time at start of first exposure; HH:MM:SS format} 
\end{deluxetable*} 


==> m2fs_obs_table.tex <==
\begin{deluxetable*}{lllllcccl} 
\tablewidth{0pt} 
\tablecaption{Log of M2FS Observations of Galactic Halo Objects \label{tab:m2fs_obs_table}} \tablehead{\colhead{Instrument}&\multicolumn{2}{l}{\colhead{Field Center}}&\colhead{UT date\tablenotemark{a}}&\colhead{UT start\tablenotemark{b}}&\colhead{Exp. Time}&\colhead{$N_{\rm exp}$}&\colhead{$N_{\rm target}$}&\colhead{Object}\\ 
&\colhead{$\alpha_{2000}$ [deg.]}&\colhead{$\delta_{2000}$ [deg.]}&&&\colhead{[sec.]}&} 
\startdata 
M2FS HiRes & $153.028333$ & $-001.754667$ & 2014-02-24 & 08:44:35 &$8900$ & $5$ & $218$ & Sextans\\ 
M2FS HiRes & $100.746667$ & $-050.848333$ & 2014-02-25 & 03:01:36 &$5400$ & $3$ & $214$ & Carina\\ 
M2FS HiRes & $100.610000$ & $-051.082361$ & 2014-02-25 & 05:04:05 &$5700$ & $3$ & $214$ & Carina\\ 
M2FS HiRes & $153.684583$ & $-001.500944$ & 2014-02-26 & 08:00:05 &$6600$ & $5$ & $216$ & Sextans\\ 
M2FS HiRes & $153.685000$ & $-001.501000$ & 2014-02-27 & 07:13:52 &$3600$ & $3$ & $216$ & Sextans\\ 
M2FS HiRes & $153.292917$ & $-001.604694$ & 2014-02-28 & 07:46:28 &$3600$ & $3$ & $216$ & Sextans\\ 
M2FS HiRes & $100.399167$ & $-050.947139$ & 2014-12-15 & 06:28:27 &$8100$ & $3$ & $218$ & Carina\\ 
M2FS HiRes & $100.835417$ & $-051.099611$ & 2014-12-19 & 08:05:29 &$4500$ & $3$ & $207$ & Carina\\ 
M2FS HiRes & $099.959583$ & $-050.786417$ & 2014-12-21 & 07:56:08 &$5400$ & $3$ & $187$ & Carina\\ 
M2FS HiRes & $099.961667$ & $-050.784722$ & 2014-12-23 & 08:01:05 &$3600$ & $3$ & $177$ & Carina\\ 
M2FS HiRes & $053.810000$ & $-054.075444$ & 2015-02-19 & 02:24:12 &$7200$ & $3$ & $186$ & Reticulum II\\ 
M2FS HiRes & $153.292500$ & $-001.601639$ & 2015-02-22 & 06:50:05 &$7200$ & $4$ & $214$ & Sextans\\ 
M2FS HiRes/MedRes & $343.062917$ & $-058.493583$ & 2015-07-18 & 09:40:45 &$9000$ & $5$ & $137$ & Tucana II\\ 
M2FS HiRes/MedRes & $344.205417$ & $-050.098472$ & 2015-07-19 & 09:15:17 &$7200$ & $3$ & $133$ & Grus I\\ 
M2FS HiRes/MedRes & $317.224583$ & $-051.240528$ & 2015-07-21 & 07:57:45 &$7200$ & $4$ & $182$ & Indus 1\\ 
M2FS HiRes/MedRes & $354.905417$ & $-054.408306$ & 2015-07-21 & 09:59:12 &$4500$ & $3$ & $158$ & Phoenix II\\ 
M2FS HiRes/MedRes & $343.059167$ & $-058.493278$ & 2015-09-13 & 02:55:30 &$8100$ & $3$ & $124$ & Tucana II\\ 
M2FS HiRes/MedRes & $343.060417$ & $-058.493833$ & 2015-09-19 & 02:49:58 &$11049$ & $4$ & $137$ & Tucana II\\ 
M2FS HiRes & $153.682917$ & $-001.498500$ & 2016-02-03 & 07:10:05 &$9000$ & $5$ & $216$ & Sextans\\ 
M2FS MedRes & $153.683333$ & $-001.498556$ & 2016-02-03 & 08:28:29 &$3600$ & $2$ & $216$ & Sextans\\ 
M2FS HiRes & $153.292083$ & $-001.602556$ & 2016-02-06 & 08:23:52 &$10500$ & $4$ & $239$ & Sextans\\ 
M2FS HiRes & $153.012500$ & $-001.195667$ & 2016-02-08 & 07:48:18 &$10800$ & $4$ & $217$ & Sextans\\ 
M2FS HiRes & $153.591250$ & $-001.235056$ & 2016-02-09 & 08:39:46 &$8400$ & $5$ & $216$ & Sextans\\ 
M2FS HiRes & $153.400000$ & $-001.850944$ & 2016-02-10 & 08:10:51 &$10800$ & $5$ & $218$ & Sextans\\ 
M2FS HiRes & $100.397917$ & $-050.947861$ & 2016-11-29 & 06:49:12 &$8100$ & $3$ & $221$ & Carina\\ 
M2FS HiRes & $100.400417$ & $-050.949167$ & 2016-11-30 & 07:39:28 &$6000$ & $2$ & $221$ & Carina\\ 
M2FS HiRes & $100.399167$ & $-050.948639$ & 2016-12-01 & 07:26:34 &$7000$ & $2$ & $220$ & Carina\\ 
M2FS HiRes & $100.398333$ & $-050.948111$ & 2016-12-02 & 07:21:25 &$8000$ & $2$ & $221$ & Carina\\ 
M2FS HiRes & $100.398750$ & $-050.948333$ & 2016-12-08 & 07:42:43 &$5400$ & $2$ & $221$ & Carina\\ 
M2FS HiRes & $100.836667$ & $-051.099694$ & 2017-03-05 & 01:51:55 &$8100$ & $3$ & $207$ & Carina\\ 
M2FS HiRes/MedRes & $343.057500$ & $-058.495889$ & 2017-05-21 & 09:50:46 &$8400$ & $3$ & $137$ & Tucana II\\ 
M2FS HiRes/MedRes & $343.059167$ & $-058.493500$ & 2017-06-02 & 09:17:16 &$12600$ & $4$ & $137$ & Tucana II\\ 
M2FS HiRes & $014.823333$ & $-033.919861$ & 2017-11-08 & 05:08:39 &$6600$ & $3$ & $238$ & Sculptor\\ 
M2FS HiRes & $100.397500$ & $-050.947694$ & 2017-11-09 & 08:09:37 &$8700$ & $3$ & $218$ & Carina\\ 
M2FS HiRes & $015.323750$ & $-033.712167$ & 2017-11-11 & 02:12:39 &$9400$ & $3$ & $238$ & Sculptor\\ 
M2FS HiRes & $014.797500$ & $-033.497667$ & 2017-11-14 & 02:02:24 &$9000$ & $3$ & $238$ & Sculptor\\ 
M2FS HiRes/MedRes & $343.059583$ & $-058.493250$ & 2017-11-20 & 01:06:58 &$4900$ & $2$ & $124$ & Tucana II\\ 
M2FS HiRes & $037.186667$ & $-079.293444$ & 2018-02-13 & 02:02:39 &$7800$ & $3$ & $235$ & Hydrus I\\ 
M2FS HiRes & $100.400000$ & $-050.948556$ & 2018-02-19 & 04:58:33 &$10000$ & $4$ & $235$ & Carina\\ 
M2FS HiRes & $101.167500$ & $-050.674889$ & 2018-05-13 & 00:16:42 &$5400$ & $3$ & $75$ & Carina\\ 
M2FS HiRes/MedRes & $343.058333$ & $-058.495528$ & 2018-05-19 & 07:51:21 &$3600$ & $2$ & $124$ & Tucana II\\ 
M2FS HiRes & $174.048750$ & $-010.941944$ & 2018-05-20 & 01:59:43 &$9900$ & $4$ & $174$ & Crater 1\\ 
M2FS HiRes & $256.135833$ & $-035.471278$ & 2018-08-11 & 02:40:32 &$6900$ & $3$ & $54$ & Gran 3\\ 
M2FS HiRes & $212.246250$ & $-065.738333$ & 2018-08-12 & 00:42:31 &$5400$ & $3$ & $205$ & Garro-01\\ 
M2FS HiRes & $278.092083$ & $-023.211194$ & 2018-08-14 & 00:42:50 &$6100$ & $3$ & $119$ & Gran 4\\ 
M2FS HiRes & $261.651250$ & $-039.280889$ & 2018-08-16 & 00:42:52 &$7200$ & $3$ & $164$ & Gaia 11\\ 
M2FS HiRes & $040.038750$ & $-034.590833$ & 2018-11-26 & 04:09:49 &$5400$ & $3$ & $232$ & Fornax\\ 
M2FS HiRes & $038.863333$ & $-034.806167$ & 2018-11-27 & 05:46:45 &$6000$ & $3$ & $172$ & Fornax\\ 
M2FS HiRes & $039.748750$ & $-034.377528$ & 2018-11-28 & 04:54:45 &$5400$ & $3$ & $232$ & Fornax\\ 
M2FS HiRes & $039.395417$ & $-035.326250$ & 2018-11-29 & 04:38:29 &$6000$ & $3$ & $232$ & Fornax\\ 
M2FS HiRes & $100.239583$ & $-051.376194$ & 2018-11-30 & 08:01:57 &$5400$ & $3$ & $224$ & Carina\\ 
M2FS HiRes & $143.857083$ & $-036.733583$ & 2018-12-01 & 07:56:49 &$5400$ & $3$ & $224$ & Antlia II\\ 
M2FS HiRes & $121.172500$ & $-038.984444$ & 2018-12-05 & 06:09:20 &$5800$ & $3$ & $56$ & Gaia 10\\ 
M2FS HiRes & $119.607083$ & $-038.984639$ & 2018-12-06 & 05:51:03 &$5400$ & $3$ & $98$ & Gaia 9\\ 
M2FS HiRes & $142.923750$ & $-035.945111$ & 2018-12-08 & 07:33:07 &$4800$ & $2$ & $216$ & Antlia II\\ 
M2FS HiRes & $144.857083$ & $-037.530833$ & 2019-02-26 & 05:43:51 &$7200$ & $3$ & $224$ & Antlia II\\ 
M2FS HiRes & $100.397917$ & $-050.948500$ & 2019-03-01 & 02:51:44 &$2400$ & $1$ & $224$ & Carina\\ 
M2FS HiRes & $100.398333$ & $-050.950139$ & 2019-03-02 & 04:28:15 &$8500$ & $4$ & $224$ & Carina\\ 
M2FS HiRes & $101.121667$ & $-050.787472$ & 2019-03-06 & 04:12:49 &$7200$ & $3$ & $224$ & Carina\\ 
M2FS HiRes & $153.026250$ & $-001.898111$ & 2019-03-06 & 06:36:48 &$5100$ & $3$ & $240$ & Sextans\\ 
M2FS HiRes & $101.122917$ & $-050.787472$ & 2019-03-07 & 02:19:11 &$8400$ & $4$ & $224$ & Carina\\ 
M2FS HiRes/MedRes & $343.062917$ & $-058.495111$ & 2019-06-02 & 10:09:54 &$2850$ & $3$ & $137$ & Tucana II\\ 
M2FS HiRes & $143.450000$ & $-037.172333$ & 2019-06-03 & 01:12:41 &$7202$ & $3$ & $224$ & Antlia II\\ 
M2FS HiRes & $143.858333$ & $-036.733722$ & 2019-06-04 & 00:45:40 &$8400$ & $3$ & $224$ & Antlia II\\ 
M2FS HiRes/MedRes & $343.058333$ & $-058.494361$ & 2019-06-04 & 09:41:46 &$5400$ & $3$ & $124$ & Tucana II\\ 
M2FS HiRes & $153.006250$ & $-001.387083$ & 2019-06-05 & 00:29:52 &$7200$ & $4$ & $240$ & Sextans\\ 
M2FS HiRes/MedRes & $343.059583$ & $-058.492139$ & 2019-06-05 & 09:39:29 &$7200$ & $4$ & $137$ & Tucana II\\ 
M2FS HiRes & $014.783750$ & $-033.924389$ & 2019-08-29 & 05:56:04 &$7900$ & $3$ & $240$ & Sculptor\\ 
M2FS HiRes & $014.891667$ & $-033.653139$ & 2019-08-30 & 05:55:41 &$7200$ & $3$ & $240$ & Sculptor\\ 
M2FS HiRes & $015.625417$ & $-033.960778$ & 2019-08-31 & 05:21:58 &$10200$ & $4$ & $233$ & Sculptor\\ 
M2FS HiRes & $040.381667$ & $-035.116361$ & 2019-08-31 & 09:17:19 &$10800$ & $4$ & $232$ & Fornax\\ 
M2FS HiRes/MedRes & $343.060417$ & $-058.495139$ & 2019-09-01 & 05:36:01 &$10200$ & $4$ & $137$ & Tucana II\\ 
M2FS HiRes & $015.265833$ & $-033.797111$ & 2019-09-02 & 06:17:59 &$9600$ & $4$ & $240$ & Sculptor\\ 
M2FS HiRes & $041.059167$ & $-033.863056$ & 2019-09-02 & 09:46:18 &$8700$ & $4$ & $141$ & Fornax\\ 
M2FS HiRes/MedRes & $343.061667$ & $-058.494917$ & 2019-09-03 & 05:43:18 &$11400$ & $4$ & $124$ & Tucana II\\ 
M2FS HiRes & $041.059583$ & $-033.862694$ & 2019-09-03 & 09:16:42 &$9600$ & $4$ & $141$ & Fornax\\ 
M2FS HiRes & $015.745000$ & $-034.255333$ & 2019-11-17 & 02:33:43 &$9420$ & $4$ & $127$ & Sculptor\\ 
M2FS HiRes & $014.268750$ & $-033.611861$ & 2019-11-18 & 02:46:52 &$10800$ & $4$ & $236$ & Sculptor\\ 
M2FS HiRes/MedRes & $343.060417$ & $-058.494944$ & 2019-11-19 & 02:39:25 &$9600$ & $4$ & $137$ & Tucana II\\ 
M2FS HiRes & $014.898750$ & $-034.173222$ & 2019-11-20 & 01:47:03 &$7800$ & $3$ & $227$ & Sculptor\\ 
M2FS HiRes & $015.492500$ & $-033.336972$ & 2019-11-21 & 01:51:48 &$8100$ & $3$ & $220$ & Sculptor\\ 
M2FS HiRes & $014.892500$ & $-033.653694$ & 2019-11-23 & 01:50:37 &$7200$ & $3$ & $240$ & Sculptor\\ 
M2FS HiRes/MedRes & $343.061250$ & $-058.494861$ & 2019-11-24 & 02:27:13 &$8700$ & $4$ & $124$ & Tucana II\\ 
M2FS HiRes & $040.323333$ & $-034.590083$ & 2019-11-24 & 05:23:20 &$6000$ & $2$ & $232$ & Fornax\\ 
M2FS HiRes & $040.242500$ & $-034.292389$ & 2020-01-27 & 02:15:16 &$6400$ & $3$ & $232$ & Fornax\\ 
M2FS HiRes & $100.395417$ & $-050.497917$ & 2020-01-27 & 05:17:55 &$8280$ & $3$ & $224$ & Carina\\ 
M2FS HiRes & $099.991250$ & $-051.038528$ & 2020-01-30 & 06:22:14 &$8700$ & $3$ & $224$ & Carina\\ 
M2FS HiRes & $153.497083$ & $-001.623556$ & 2020-01-31 & 08:32:48 &$9500$ & $4$ & $240$ & Sextans\\ 
M2FS HiRes & $099.734583$ & $-050.822667$ & 2020-02-03 & 06:37:52 &$7800$ & $3$ & $224$ & Carina\\ 
M2FS HiRes & $343.060417$ & $-058.493222$ & 2022-05-27 & 09:55:22 &$5400$ & $3$ & $132$ & Tucana II\\ 
M2FS HiRes & $039.305000$ & $-033.763583$ & 2022-11-20 & 02:32:39 &$9720$ & $3$ & $116$ & Fornax\\ 
M2FS HiRes & $040.329167$ & $-033.587694$ & 2022-11-21 & 02:44:48 &$7200$ & $3$ & $207$ & Fornax\\ 
\enddata 
\tablenotetext{a}{YYYY-MM-DD format} 
\tablenotetext{b}{Universal time at start of first exposure; HH:MM:SS format} 
\end{deluxetable*} 


==> offsets.tex <==
\newcommand{\mtwofshireshectovn}{199} 
\newcommand{\mtwofshireshthreevn}{87} 
\newcommand{\mtwofshireswalkervn}{1489} 
\newcommand{\mtwofshiresapogeevn}{136} 
\newcommand{\mtwofshiresssppvn}{1037} 
\newcommand{\mtwofshiresmtwofsmedresvn}{29} 
\newcommand{\mtwofshiresgaiavn}{5} 
\newcommand{\hectohthreevn}{767} 
\newcommand{\hectowalkervn}{194} 
\newcommand{\hectoapogeevn}{116} 
\newcommand{\hectossppvn}{2753} 
\newcommand{\hectomtwofsmedresvn}{5} 
\newcommand{\hectogaiavn}{48} 
\newcommand{\hthreewalkervn}{91} 
\newcommand{\hthreeapogeevn}{30} 
\newcommand{\hthreemtwofsmedresvn}{2} 
\newcommand{\hthreegaiavn}{426} 
\newcommand{\walkerapogeevn}{281} 
\newcommand{\walkermtwofsmedresvn}{11} 
\newcommand{\walkergaiavn}{3666} 
\newcommand{\mtwofsmedresapogeevn}{2} 
\newcommand{\mtwofsmedresgaiavn}{1} 
\newcommand{\gaiaapogeevn}{341914} 
\newcommand{\mtwofshireshectoteffn}{199} 
\newcommand{\mtwofshireskirbyteffn}{117} 
\newcommand{\mtwofshireshthreeteffn}{87} 
\newcommand{\mtwofshiresapogeeteffn}{136} 
\newcommand{\mtwofshiresssppteffn}{1037} 
\newcommand{\mtwofshiresmtwofsmedresteffn}{29} 
\newcommand{\mtwofshiresgaiateffn}{5} 
\newcommand{\hectokirbyteffn}{326} 
\newcommand{\hectohthreeteffn}{767} 
\newcommand{\hectoapogeeteffn}{116} 
\newcommand{\hectossppteffn}{2753} 
\newcommand{\hectomtwofsmedresteffn}{5} 
\newcommand{\hectogaiateffn}{48} 
\newcommand{\kirbyhthreeteffn}{25} 
\newcommand{\kirbyapogeeteffn}{79} 
\newcommand{\kirbygaiateffn}{490} 
\newcommand{\hthreeapogeeteffn}{30} 
\newcommand{\hthreemtwofsmedresteffn}{2} 
\newcommand{\hthreegaiateffn}{426} 
\newcommand{\mtwofsmedresapogeeteffn}{2} 
\newcommand{\m2fsmedresgaiateffn}{1} 
\newcommand{\gaiaapogeeteffn}{341914} 
\newcommand{\mtwofshireshectologgn}{199} 
\newcommand{\mtwofshireskirbyloggn}{117} 
\newcommand{\mtwofshireshthreeloggn}{87} 
\newcommand{\mtwofshiresapogeeloggn}{136} 
\newcommand{\mtwofshiressspploggn}{1037} 
\newcommand{\mtwofshiresmtwofsmedresloggn}{29} 
\newcommand{\mtwofshiresgaialoggn}{1} 
\newcommand{\hectokirbyloggn}{326} 
\newcommand{\hectohthreeloggn}{767} 
\newcommand{\hectoapogeeloggn}{116} 
\newcommand{\hectosspploggn}{2753} 
\newcommand{\hectomtwofsmedresloggn}{5} 
\newcommand{\hectogaialoggn}{48} 
\newcommand{\kirbyhthreeloggn}{25} 
\newcommand{\kirbyapogeeloggn}{79} 
\newcommand{\kirbygaialoggn}{490} 
\newcommand{\hthreeapogeeloggn}{30} 
\newcommand{\hthreemtwofsmedresloggn}{2} 
\newcommand{\hthreegaialoggn}{426} 
\newcommand{\mtwofsmedresapogeeloggn}{2} 
\newcommand{\mtwofsgaialoggn}{1} 
\newcommand{\gaiaapogeeloggn}{341914} 
\newcommand{\mtwofshireshectofehn}{199} 
\newcommand{\mtwofshireskirbyfehn}{117} 
\newcommand{\mtwofshireshthreefehn}{87} 
\newcommand{\mtwofshiresapogeefehn}{136} 
\newcommand{\mtwofshiresssppfehn}{1037} 
\newcommand{\mtwofshiresmtwofsmedresfehn}{29} 
\newcommand{\mtwofshiresgaiafehn}{5} 
\newcommand{\hectokirbyfehn}{326} 
\newcommand{\hectohthreefehn}{767} 
\newcommand{\hectoapogeefehn}{116} 
\newcommand{\hectossppfehn}{2753} 
\newcommand{\hectomtwofsmedresfehn}{5} 
\newcommand{\hectogaiafehn}{48} 
\newcommand{\kirbyhthreefehn}{25} 
\newcommand{\kirbyapogeefehn}{79} 
\newcommand{\kirbygaiafehn}{490} 
\newcommand{\hthreeapogeefehn}{30} 
\newcommand{\hthreemtwofsmedresfehn}{2} 
\newcommand{\hthreegaiafehn}{426} 
\newcommand{\mtwofsmedresapogeefehn}{2} 
\newcommand{\mtwofsgaiafehn}{1} 
\newcommand{\gaiaapogeefehn}{341914} 
\newcommand{\mtwofshireshectoalphan}{199} 
\newcommand{\mtwofshireskirbyalphan}{117} 
\newcommand{\mtwofshireshthreealphan}{87} 
\newcommand{\mtwofshiresapogeealphan}{136} 
\newcommand{\mtwofshiresmtwofsmedresalphan}{29} 
\newcommand{\hectokirbyalphan}{326} 
\newcommand{\hectohthreealphan}{767} 
\newcommand{\hectoapogeealphan}{116} 
\newcommand{\hectomtwofsmedresalphan}{5} 
\newcommand{\kirbyhthreealphan}{25} 
\newcommand{\kirbyapogeealphan}{79} 
\newcommand{\hthreeapogeealphan}{30} 
\newcommand{\hthreemtwofsmedresalphan}{2} 
\newcommand{\mtwofsmedresapogeealphan}{2} 
\newcommand{\mtwofshiresvoffset}{$0.56\pm 0.05$} 
\newcommand{\hectovoffset}{$-0.15\pm 0.04$} 
\newcommand{\kirbyvoffset}{$-0.04\pm 2.90$} 
\newcommand{\hthreevoffset}{$-0.29\pm 0.05$} 
\newcommand{\walkervoffset}{$-0.20\pm 0.05$} 
\newcommand{\mtwofsmedresvoffset}{$1.25\pm 0.27$} 
\newcommand{\gaiavoffset}{$0.05\pm 2.85$} 
\newcommand{\mtwofshiresteffoffset}{$-133\pm 6$} 
\newcommand{\hectoteffoffset}{$-213\pm 3$} 
\newcommand{\kirbyteffoffset}{$-171\pm 2$} 
\newcommand{\hthreeteffoffset}{$-60\pm 3$} 
\newcommand{\walkerteffoffset}{$-1\pm 286$} 
\newcommand{\mtwofsmedresteffoffset}{$-282\pm 27$} 
\newcommand{\gaiateffoffset}{$12\pm 283$} 
\newcommand{\mtwofshiresloggoffset}{$-0.54\pm 0.02$} 
\newcommand{\hectologgoffset}{$-0.48\pm 0.01$} 
\newcommand{\kirbyloggoffset}{$-0.27\pm 0.01$} 
\newcommand{\hthreeloggoffset}{$-0.22\pm 0.01$} 
\newcommand{\walkerloggoffset}{$0.02\pm 0.56$} 
\newcommand{\mtwofsmedresloggoffset}{$-0.33\pm 0.06$} 
\newcommand{\gaialoggoffset}{$0.02\pm 0.58$} 
\newcommand{\mtwofshiresfehoffset}{$-0.26\pm 0.01$} 
\newcommand{\hectofehoffset}{$-0.26\pm 0.01$} 
\newcommand{\kirbyfehoffset}{$-0.17\pm 0.01$} 
\newcommand{\hthreefehoffset}{$-0.01\pm 0.01$} 
\newcommand{\walkerfehoffset}{$0.02\pm 0.57$} 
\newcommand{\mtwofsmedresfehoffset}{$-0.39\pm 0.04$} 
\newcommand{\gaiafehoffset}{$-0.02\pm 0.57$} 
\newcommand{\mtwofshiresalphaoffset}{$0.18\pm 0.01$} 
\newcommand{\hectoalphaoffset}{$-0.01\pm 0.01$} 
\newcommand{\kirbyalphaoffset}{$0.23\pm 0.02$} 
\newcommand{\hthreealphaoffset}{$0.21\pm 0.01$} 
\newcommand{\walkeralphaoffset}{$0.00\pm 0.58$} 
\newcommand{\mtwofsmedresalphaoffset}{$-0.03\pm 0.03$} 


==> weird_newcommands.tex <==
\newcommand{\mtwofsphotvariablen}{$620$} 
\newcommand{\mtwofsphotvariablegoodn}{$352$} 
\newcommand{\mtwofsrrln}{$448$} 
\newcommand{\mtwofsrrlgoodn}{$301$} 
\newcommand{\mtwofscepheidn}{$0$} 
\newcommand{\mtwofscepheidgoodn}{$0$} 
\newcommand{\mtwofsagnn}{$105$} 
\newcommand{\mtwofsagngoodn}{$81$} 
\newcommand{\mtwofsrvvariablen}{$0$} 
\newcommand{\mtwofsrvvariablegoodn}{$0$} 
\newcommand{\mtwofscompactcompanionn}{$0$} 
\newcommand{\mtwofscompactcompaniongoodn}{$0$} 
\newcommand{\mtwofschitwooutliern}{$90$} 
\newcommand{\mtwofschitwooutliergoodn}{$51$} 
\newcommand{\mtwofscarbonn}{$336$} 
\newcommand{\mtwofscarbongoodn}{$38$} 
\newcommand{\hectophotvariablen}{$861$} 
\newcommand{\hectophotvariablegoodn}{$78$} 
\newcommand{\hectorrln}{$302$} 
\newcommand{\hectorrlgoodn}{$37$} 
\newcommand{\hectocepheidn}{$0$} 
\newcommand{\hectocepheidgoodn}{$0$} 
\newcommand{\hectoagnn}{$422$} 
\newcommand{\hectoagngoodn}{$369$} 
\newcommand{\hectorvvariablen}{$0$} 
\newcommand{\hectorvvariablegoodn}{$0$} 
\newcommand{\hectocompactcompanionn}{$0$} 
\newcommand{\hectocompactcompaniongoodn}{$0$} 
\newcommand{\hectochitwooutliern}{$251$} 
\newcommand{\hectochitwooutliergoodn}{$130$} 
\newcommand{\hectocarbonn}{$1466$} 
\newcommand{\hectocarbongoodn}{$143$} 

